From Latent Biomarkers to Clinical Rules: Embedding-Guided Rule Mining and Attribution-Based Translation for Interpretable Tabular Learning

Clinical decision support tools are most useful when accurate predictions are accompanied by understandable explanations. Rule-based models provide transparency, but rules derived directly from raw clinical measurements may miss patterns arising from interactions between multiple variables. We present a four-step pipeline that mines decision rules in the latent space of an FT-Transformer and translates them back into measurable clinical features. Embedding dimensions that consistently separate patient groups are treated as latent biomarkers, rules are mined using small decision trees, and selected rules are translated using gradient-input saliency and CLS attention attribution. We evaluate the framework on six public clinical and population health datasets at four embedding dimensions. Translated rules outperformed raw-feature rules in five of six datasets, with mean AUROC gains ranging from 0.04 to 0.23. On the heart disease dataset, embedding-space rules reached 0.98 AUROC, but translation reduced this to 0.72, showing that high-performing latent rules cannot always be represented by simple raw-feature conditions. These results show that latent-space rule discovery can uncover predictive patterns while translating them into clinically measurable features that can be evaluated by clinicians.

==> sections/old.tex <==
%% 01_introduction.tex

\section{Introduction}
\label{sec:introduction}

Clinicians rarely make diagnostic decisions based on a single measurement.
A diagnosis of alcoholic liver disease, the risk of hospital readmission in
a diabetic patient, or the likelihood of a cardiac event all depend on reading
multiple clinical indicators together, each individually incomplete.
Clinical decision support systems are designed to assist this process by
providing structured guidance derived from patient data, and the format that
physicians most readily adopt is the explicit IF-THEN rule.
A statement such as ``if fasting glucose exceeds 126~mg/dL and BMI is above
30~kg/m\textsuperscript{2}, flag for diabetes screening'' is transparent,
auditable, and can be embedded directly into an electronic health record (EHR)
workflow without requiring clinicians to treat the system as a black box.

The standard way to generate such rules is to train a decision tree directly
on measured feature values.
This is reliable and well understood, but it carries a structural limitation:
each split acts on a single feature at a time, and the features are used
exactly as they appear in the patient record.
Patterns that require multiple variables to interact, or that are partly
obscured by measurement noise and scale differences, are difficult to capture
by greedy splits on raw values.
Rules built this way often show acceptable performance on the training
population but generalize poorly, particularly in datasets where class
imbalance, missing values, or many weakly predictive features are present.

Transformer architectures adapted for tabular inputs have substantially
changed what is achievable in this space.
The Feature Tokenizer and Transformer~\citep{gorishniy2021} projects each
clinical measurement, whether a continuous laboratory value, a categorical
symptom grade, or a binary indicator, into a shared token representation and
processes all features jointly through multi-head self-attention.
The resulting patient representation, a compact vector in a learned latent
space, encodes feature interactions that individual measurements do not reveal
on their own.
On tabular benchmarks covering a range of clinical domains, this architecture
matches or surpasses gradient-boosted tree ensembles when sufficient training
data are available~\citep{grinsztajn2022,shwartzziv2022}.

The latent representation itself is not interpretable.
A patient described as a 32-dimensional vector, or a rule that says
``$z_3 > 0.52$ predicts high disease severity,'' conveys nothing that
a clinician can use or evaluate.
Deploying such a rule directly in a hospital would require unconditional trust
in a system whose reasoning is invisible, which conflicts with patient safety
requirements and the ethical standards of evidence-based medicine
\citep{rudin2019,ghassemi2021}.

The work presented here bridges this gap.
We propose treating the embedding dimensions that most strongly separate
patient groups as \textit{latent biomarkers}: hidden surrogates of disease
state that the model has learned to extract from the raw clinical variables.
In the same way that serum creatinine serves as a surrogate for kidney
function without directly measuring glomerular filtration rate, a latent
biomarker is a derived indicator whose discriminative power reflects an
underlying disease process captured by the model.
Decision rules are mined in this latent biomarker space, where class-relevant
structure is cleaner and more compact than in raw-feature space.
Each selected rule is then attributed back to raw clinical features using
gradient saliency and CLS attention weights from the transformer itself,
producing a translated rule that is again written in terms that appear in
a patient's chart.
Figure~\ref{fig:concept} illustrates the overall approach.

\begin{figure*}[t]
  \centering
  \includegraphics[width=\linewidth]{figures/fig_conceptual overview.png}
  \caption{Conceptual overview of the proposed pipeline. Clinical patient
  records are encoded into a compact latent space by a trained FT-Transformer
  (forward path, blue). Interpretable rules are mined in the latent space and
  the embedding dimensions involved are identified as latent biomarkers.
  Gradient and attention attribution then maps each rule back to raw clinical
  features, producing a translated rule in clinical language (attribution
  path, red).}
  \label{fig:concept}
\end{figure*}

This paper makes three contributions.
First, we formalize the concept of latent biomarkers for tabular clinical data:
embedding dimensions are ranked by their AUROC when used as a one-dimensional
predictor, and those that pass a confidence and coverage threshold in the
extracted rules are designated as biomarkers for the corresponding outcome
class.
Second, we describe a combined attribution method that translates
embedding-space rules into raw-feature conditions by aggregating
gradient-input saliency across all latent dimensions in a rule and weighting
it with CLS attention scores, then fitting a shallow decision tree on the
top-ranked raw features.
Third, we evaluate the complete framework on six publicly available clinical
datasets spanning hepatic, cardiac, and metabolic disease domains, and
demonstrate that translated rules outperform raw-feature rules in five of
six cases, with AUROC gains reaching 0.22 in the largest datasets.

The rest of the paper is organized as follows.
Section~\ref{sec:related} reviews related work on transformer models for
tabular data, interpretable machine learning, and attribution methods.
Section~\ref{sec:methods} describes the datasets and the four-step pipeline
in detail.
Section~\ref{sec:results} presents the performance comparisons.
Section~\ref{sec:discussion} discusses the findings and their clinical
implications.
Section~\ref{sec:conclusion} concludes.

